LUCID: Learning-Enabled Uncertainty-Aware Certification of Stochastic Dynamical Systems

Ensuring the safety of AI-enabled systems, particularly in high-stakes domains such as autonomous driving and healthcare, has become increasingly critical. Traditional formal verification tools fall short when faced with systems that embed both opaque, black-box AI components and complex stochastic dynamics. To address these challenges, we introduce LUCID (Learning-enabled Uncertainty-aware Certification of stochastIc Dynamical systems), a verification engine for certifying safety of black-box stochastic dynamical systems from a finite dataset of random state transitions. As such, LUCID is the first known tool capable of establishing quantified safety guarantees for such systems. Thanks to its modular architecture and extensive documentation, LUCID is designed for easy extensibility. LUCID employs a data-driven methodology rooted in control barrier certificates, which are learned directly from system transition data, to ensure formal safety guarantees. We use conditional mean embeddings to embed data into a reproducing kernel Hilbert space (RKHS), where an RKHS ambiguity set is constructed that can be inflated to robustify the result to out-of-distribution behavior. A key innovation within LUCID is its use of a finite Fourier kernel expansion to reformulate a semi-infinite non-convex optimization problem into a tractable linear program. The resulting spectral barrier allows us to leverage the fast Fourier transform to generate the relaxed problem efficiently, offering a scalable yet distributionally robust framework for verifying safety. LUCID thus offers a robust and efficient verification framework, able to handle the complexities of modern black-box systems while providing formal guarantees of safety. These unique capabilities are demonstrated on challenging benchmarks.

==> glossary.tex <==
\newglossaryentry{oop}{
    name={Object-Oriented Programming},
    first={Object-Oriented Programming (OOP)},
    text={OOP},
    description={
            Object-Oriented Programming is a programming paradigm based on the concept of objects, which can hold a state in the form of fields, and methods, in the form of function with access to the object's state.
        }
}
\newglossaryentry{api}{
    name = {Application Programming Interface},
    first = {Application Programming Interface (API)},
    text = {API},
    plural={APIs},
    firstplural={Application Programming Interfaces (APIs)},
    description = {
            An application programming interface (API) defines a way for two software components to communicate with each other.
        }
}
\newglossaryentry{smt}
{
    name={Satisfiability Modulo Theories},
    first={Satisfiability Modulo Theories (SMT)},
    text={SMT},
    description={
            A decision problem for logical formulas with respect to combinations of background theories
            expressed in classical first-order logic with equality.
        }
}
\newglossaryentry{fol}{
    name={First-order logic},
    first={first-order logic (FOL)},
    text={fol},
    description={
            Expressive formal system that allows the following statements:
            \begin{itemize}
                \item Constants ($x, y$)
                \item Functions ($f(x)$)
                \item Relationships ($x > y$)
                \item Connectives ($\land, \lor, \lnot, \implies, \iff$)
                \item Quantifiers ($\forall, \exists$)
            \end{itemize}
        }
}
\newglossaryentry{smtp}{
    name={SMT problem},
    text={SMT problem},
    plural={SMT problems},
    description={
            Decision problems that are true or false depending on whether a given \gls{fol} formula
            is true or false in respect to a given background theory. \\
            In the context of computer science, the background theories are usually include
            arithmetic, bitvectors, arrays, etc.
        }
}
\newglossaryentry{sat}{
    first={Satisfiability (SAT)},
    name={Satisfiability},
    text={SAT},
    description={
            A formula is satisfiable if it is possible to find a set of values for its variables
            that makes the formula true.
            On the other hand, a formula is unsatisfiable if such set does not exists.
            \begin{multline*}
                \text{Example} \\
                (a \lor c) \land (b \lor c) \land (\neg a \lor \neg c) \\
                \text{is satisfiable with the assignment } a = 1, b = 1, c = 0 \\
            \end{multline*}
        }
}
\newglossaryentry{convopt}{
    name={Convex optimization},
    text={convex optimization},
    description={
            A convex optimization problem is a problem where the objective function and the constraints
            are convex functions. \\
            A convex function is a function whose domain is a convex set and that satisfies the following
            property:
            \begin{equation*}
                f(\lambda x + (1 - \lambda)y) \leq \lambda f(x) + (1 - \lambda)f(y)
            \end{equation*}
            for all $x, y \in \text{dom}(f)$ and $\lambda \in [0, 1]$.
        }
}
\newglossaryentry{cnf}{
    first={Conjunctive Normal Form (CNF)},
    name={Conjunctive Normal Form},
    text={CNF},
    description={
            A formula is in \gls{cnf} if it is a conjunction of clauses, where a clause is a
            disjunction of literals. \\
            A literal can be a boolean variable or its negation. \\
            \\
            \begin{equation*}
                \bigwedge_{i=1}^n \bigvee_{j=1}^{m_i} l_{ij}
            \end{equation*}
        }
}
\newglossaryentry{lp}{
    first={Linear Program (LP)},
    name={Linear Program},
    text={LP},
    description={
            A Linear Program is an optimization problem where the objective function and the constraints
            are linear functions. \\
            A typical Linear Program has the following form:
            \begin{equation*}
                \begin{aligned}
                     & \text{maximize}   & c^T x      \\
                     & \text{subject to} & A x \leq b \\
                     &                   & x \geq 0
                \end{aligned}
            \end{equation*}
            where $x \in \mathbb{R}^d$ is the vector of variables to be determined, $c \in \mathbb{R}^d$ and $b \in \mathbb{R}^n$ are vectors of coefficients, and $A \in \mathbb{R}^{n \times d}$ is a matrix of coefficients.
        }
}
\newglossaryentry{qf-lia}{
    name={QF\_LIA},
    text={QF\_LIA},
    description={
            Quantifier-free linear integer arithmetic. In essence, Boolean combinations of inequations between linear polynomials over integer variables.
        }
}
\newglossaryentry{qf-lra}{
    name={QF\_LRA},
    text={QF\_LRA},
    description={
            Quantifier-free linear real arithmetic. In essence, Boolean combinations of inequations between linear polynomials over real variables.
        }
}
\newglossaryentry{nnf}{
    name={Negation Normal Form},
    text={NNF},
    first={Negation Normal Form (NNF)},
    description={
            A formula where the negation operator $\neg$ is only applied to variables. \\
            $\neg a$ is a NNF formula, while $\neg (a \lor b)$ is not.
        }
}
\newglossaryentry{dpll}{
    name={DPLL algorithm},
    text={DPLL},
    first={Davis-Putnam-Logemann-Loveland (DPLL)},
    description={
            A complete \gls{sat} backtracking algorithm for deciding the satisfiability of propositional logic formulae in \gls{cnf}.
        }
}
\newglossaryentry{dp}{
    name={DP algorithm},
    text={DP},
    first={Davis-Putnam (DP)},
    description={
            A complete \gls{sat} algorithms that uses the resolution inference rule to decide the satisfiability of propositional logic formulae in \gls{cnf}.
        }
}
\newglossaryentry{mps}{
    name={Mathematical Programming System},
    text={MPS},
    first={Mathematical Programming System (MPS)},
    description={
            A common file format for representing \gls{lp} problems.
            Developed by IBM, it is supported by most commercial \gls{lp} solvers.
        }
}
\newglossaryentry{soi}{
    name={Sum of Infeasibilities},
    text={SoI},
    first={Sum of Infeasibilities (SoI)},
    description={
            A metric used to evaluate the quality of an \gls{lp} relaxation.
            It is the sum of the infeasibilities of the constraints that are violated by the solution.
        }
}
\newglossaryentry{onnx}{
    name={Open Neural Network Exchange},
    text={ONNX},
    first={Open Neural Network Exchange (ONNX)},
    description={
            An open-source format for representing deep learning models.
            It is supported by a wide range of tools and libraries.
        }
}
\newglossaryentry{cdlc}{
    name={Conflict Driven Learning Clause},
    text={CDLC},
    first={Conflict Driven Learning Clause (CDLC)},
    description={
            A clause that is added to the \gls{cnf} formula after a conflict is detected during the \gls{sat} solving process.
            It is used to prevent the solver from exploring the same path that led to the conflict.
        }
}
\newglossaryentry{rkhs}{
    name={Reproducing Kernel Hilbert Space},
    text={RKHS},
    first={Reproducing Kernel Hilbert Space (RKHS)},
    firstplural={Reproducing Kernel Hilbert Spaces (RKHS)},
    description={}
}
\newglossaryentry{cbc}{
    name={Control Barrier Certificate},
    text={CBC},
    plural={CBCs},
    first={\emph{Control Barrier Certificate} (CBC)},
    firstplural={\emph{Control Barrier Certificates} (CBCs)},
    description={}
}
\newglossaryentry{cbf}{
    name={Control Barrier Certificate},
    text={CBF},
    plural={CBFs},
    first={\emph{Control Barrier Function} (CBF)},
    firstplural={\emph{Control Barrier Functions} (CBFs)},
    description={}
}
\newglossaryentry{gui}{
    name={Graphical User Interface},
    text={GUI},
    first={\emph{Graphical User Interface} (GUI)},
    description={}
}
\newglossaryentry{cli}{
    name={Command Line Interface},
    text={CLI},
    first={\emph{Command Line Interface} (CLI)},
    description={}
}
\newglossaryentry{nn}{
    name={Neural Network},
    text={NN},
    first={Neural Network (NN)},
    firstplural={Neural Networks (NNs)},
    description={}
}
\newglossaryentry{cme}{
    name={Conditional Mean Embedding},
    text={CME},
    plural={CMEs},
    first={\emph{Conditional Mean Embedding} (CME)},
    firstplural={\emph{Conditional Mean Embeddings} (CMEs)},
    description={}
}
\newglossaryentry{rl}{
    name={Reinforcement Learning},
    text={RL},
    first={Reinforcement Learning (RL)},
    description={}
}
\newglossaryentry{mdp}{
    name={Markov Decision Process},
    text={MDP},
    plural={MDPs},
    first={Markov Decision Process (MDP)},
    firstplural={Markov Decision Processes (MDPs)},
    description={}
}

